Diversity-Multiplexing Tradeoff in Fading Interference Channels

We analyze two-user single-antenna fading interference channels with perfect receive channel state information (CSI) and no transmit CSI. We compute the diversity-multiplexing tradeoff (DMT) region of a fixed-power-split Han and Kobayashi (HK)-type superposition coding scheme and provide design criteria for the corresponding superposition codes. We demonstrate that this scheme is DMT-optimal under moderate, strong, and very strong interference by showing that it achieves a DMT outer bound that we derive. Further, under very strong interference, we show that a joint decoder is DMT-optimal and "decouples" the fading interference channel, i.e., from a DMT perspective, it is possible to transmit as if the interfering user were not present. In addition, we show that, under very strong interference, decoding interference while treating the intended signal as noise, subtracting the result out, and then decoding the desired signal, a process known as "stripping", achieves the optimal DMT region. Our proofs are constructive in the sense that code design criteria for achieving DMT-optimality (in the cases where we can demonstrate it) are provided.

==> Makefile <==
# LaTeX Makefile for use with the CTGTeX workflow
# generated Wed, 06, May, 2009 00:31:45UTC

# project directory: /Users/akcabac/Desktop/ArxivJournal
# project name, i.e., name of master latex file without ".tex" extension
PROJ = intjour

# additional (.tex) files that LaTeX depends on, i.e.macro files
AUX = cakcaba-macros.tex 

# graphics files used by \includegraphics
FIGS = onesided.pdf div05.pdf div066.pdf div1.pdf div15.pdf 

# set to nonempty value to enable BibTeX
USEBIBTEX = 1

# is .bbl file in CVS? Leave blank if no, set to 1 if .bbl in CVS.
# If set to 1, bibtex won't be run (in order not to clobber the .bbl file).
BBLINCVS = 

# include master makefile
include $(CTGTEXDIR)/scripts/Pdflatex.mk

